Narrative Keyframing for Generative Creative Writing

We introduce narrative keyframing, an interaction technique for AI-assisted creative writing that lets writers specify different types of narrative constraints at selected moments in a story, then use AI to generate intervening prose. Inspired by the use of keyframing in animation, narrative keyframing offers a flexible way to connect story planning with adaptive control over generated text. We explore three types of keyframes: plot keyframes define significant events in a story, character keyframes represent how individual characters change over the narrative, and perspective keyframes capture how individual characters experience different events through first-person narratives. Plot and character keyframes offer a flexible way to adapt the type of high-level conditioning explored in previous AI writing tools to more customizable, iterative, and fine-scale control, while perspective keyframes add a new way to control characterization and focalization by using first-person narratives as an intermediary. Through a user study, we show that narrative keyframing supports a more controllable, transparent, and engaging way to use generative AI in creative writing.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> figures/fig-reviewpanel.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/review_panel.jpg}
  \caption{\formatcaption{Review panel.}{...}}
  \Description{}
  \label{fig:review_panel}
  % \vspace{-20pt}
\end{figure}

==> figures/fig-views.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{figures/views.pdf}
  \caption{\formatcaption{Table View and Canvas View.}{The (A) Table view presents the plot outline, each character's first-person perspective, and the generated third-person narrative side by side. This allows writers to compare them in parallel and trace how details from the outline and perspectives are transformed into the final narrative. The (B) Canvas view supports broader exploration by allowing writers to create multiple character arcs for a single character and combine different arcs across characters to generate alternative versions of the final narrative.}}
  \Description{}
  \label{fig:views}
  % \vspace{-20pt}
\end{figure*}

==> sections/1-introduction.tex <==
\section{Introduction}

% \vspace{0.2cm}
% \begin{quote}
% \small{\textit{
% ``The speciality of the novel is that the writer can talk about his characters as well as through them or can arrange for us to listen when they talk to themselves."}}\\[3pt]
% \scriptsize{\rightline{--- Edward Morgan Forster\hspace{1.2cm}}\\
% \rightline{``Aspects of The Novel", 1927 \cite{forsterAspectsNovel1927}\hspace{1.2cm}}}
% \end{quote}



%%%%%%%%%
% \noindent{}

In animation, the practice of keyframing offers an incredibly flexible and efficient way to balance automation with creative control. The basic idea is simple: most of the important detail in an animation can be derived from constraints on a sparse set of key moments. By letting users control the type and distribution of such constraints across a timeline, they can focus creative effort where it is most necessary and leverage automation where it is most appropriate.

Creative writing often follows a similar workflow, with writers planning out key moments in a story before connecting those moments with actual prose. In literary theory, this can be described as developing \newterm{plot}, which encompasses the core events of a story, before \newterm{narrative}, which encompasses how those events are presented to the reader~\cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}. 

Recent AI writing systems have leveraged high-level story descriptions, character specifications, or outlines of plot to condition the generation of narrative prose (\eg \cite{qinCharacterMeetSupportingCreative2024,schmittCharacterChatSupportingCreation2021,mirowskiCoWritingScreenplaysTheatre2023}). However, these systems typically treat such conditions as static prompts or global planning artifacts, failing to offer the kind of adaptable control afforded by animation keyframes. 




\abe{CONNECT THE ABOVE WITH THE MISSING BITS THAT ARE IN THE OLD VERSION (e.g., what we do and what our contributions are)}


% Writers often need more localized control: introducing additional structure around difficult scenes while leaving routine transitions unspecified, refining individual character arcs independently, or revisiting specific portions of a story without redefining the entire plan. Existing interfaces provide limited support for this adaptive allocation of authorial control.


% For readers, plot is accessible only through narrative. During writing, however, this relationship is often reversed: authors first construct a sequence of plot points, then develop and connect those points through narrative.




% so by letting artists focusing their creative efforts on those moments (literally, ``key frames'') and letting some other process (human, computer, etc.)













% to  of keyframes can be varied to adjusted to control the level of fine-scale control  at different points on a timeline. Each keyframe offers local control over a given property, and the distribution of keyframes over a timeline localizes control over a given property, and more Artists can add or remove different keyframe types to adaThis provides a flexible way to balance automation with creative control, as artists can By adjusting the density of each keyframe type across a timeline artists can      input  across a  the  technique for using computation to automate the interpolation artistic decisions across a timeline into a more When computers entered the picture, this workflow was adapted for digital animation by letting computers interpolate the properties of computer graphics. Modern computer animation generalizes the this approach to let different types of keyframes asynchronously control different properties of an animation (e.g. position, rotation, or scale). 

% keyframes In all of these iterations, the basic motivation of keyframing has remained the same: 


% With digital tools, artists can specify different types of keyframes (e.g., position, rotation, scale) to automate the control of  different properties. 

% Modern animation  with different types of keyframes used to control  different properties in parallel. The basic motivation for keyframes remains the same: most of the important detail in an animation can be derived from the definition of certain key moments on a timeline, so an ideal workflow should only require artists to specify those moments. Keyframes offer a flexible way to specify such moments, as keyframes can always be added or removed to adjust the level of detailed control over different parts of a an animation.


Creative writing is often discussed at two complementary levels: \newterm{plot}, which encompasses the core events of a story, their causal relationships, and the order in which they occur; and \newterm{narrative}, which describes the voice and manner in which the story is told \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}. For readers, plot is accessible only through narrative. During the writing process, however, this relationship is often reversed: authors begin by constructing a sequence of plot points, then use narrative to develop and connect those points in prose. This top-down approach helps writers externalize and iterate on plot-level decisions before investing in specific prose, and enables techniques like foreshadowing by letting earlier narrative be written with full knowledge of events that have not yet been revealed to the reader.
In this top-down workflow, planned plot points (sometimes called ``beats'') provide structural anchors from which intervening narrative can be derived. In this way, the function of planned plot points is similar to that of keyframes in animation. Motivated by this observation, we introduce a technique for AI-assisted writing based on what we call \textit{narrative keyframes}. Just as keyframes in animation let artists specify key changes to different animation properties across a timeline, narrative keyframes let authors specify key changes to different narrative properties across a plot. 

% Our prototype system offers control through three \emph{plot keyframes} define significant events in a story, \emph{character keyframes} represent how individual characters change over the narrative, and \emph{perspective keyframes} capture how individual characters experience different events through first-person narratives.

Our work offers two main contributions. The first comes from introducing narrative keyframes as a means of controlling AI-generated prose. While previous work has explored the use of plot and character constraints to control generated prose, our use of keyframes generalizes this by letting users selectively adapt the level of detail for control at different points in a narrative. This new ability to localize narrative control then motivates our second contribution, which involves the use of perspective keyframes to control characterization and focalization in generated prose. 

by changing the number and placement of keyframes. the lecel of  and localize constraints to adapt the . And second, apply more constraints for finer-scale control over  around certain parts of the narrative by defining  the level of selectively specify more keyframes where finer-scale control over the narrative is desired.  contribution extends the type of narrative conditioning  explored in previous systems 

% that define . : high-level representations of narrative that offer 
% plot events, character arcs, and narrative perspective designed to help plan and guide generative creative writing.



Motivated by these observations, we introduce a system for AI-assisted writing based on \textit{narrative keyframes}: high-level representations of plot events, character arcs, and narrative perspective designed to help plan and guide generative creative writing. Narrative keyframes let writers define character arcs that unfold in parallel with the story's overarching plot, use those arcs to guide the generation of narrative text from the perspective of different characters, then recombine elements from across those different perspectives to guide characterization and focalization in newly generated text. We evaluate our approach through a technical assessment that combines automatic metrics and expert judgments, as well as a user study with 12 writers. Results show that our system produces stories with higher overall quality and richer characterization than a standard LLM baseline, and supports a more controllable, transparent, and engaging writing experience.

\todo{
- Revise Introduction to more clearly emphasize our focus on characterization and better introduce the two innovations: keyframing metaphor and the use of first-person perspective.
}

\input{figures/fig-analogy}

% the act of planning out plot points (sometimes called ``beats'') performs a function similar to keyframing in animation by providing structural anchors from which intervening narrative can be derived. However, narrative does much more than interpolate between these anchors: it fundamentally shapes how readers perceive characters, events, and meaning, which is why the same plot can feel radically different depending on whose perspective it inhabits and how that perspective is rendered.

% \noindent{}Creative writing is often discussed at two complementary levels: \newterm{plot}, which encompasses the core events of a story, their causal relationships, and the order in which they occur; and \newterm{narrative}, which describes the voice and manner in which the story is told \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}. Distinguishing between these levels provides a useful lens for looking at the structure of creative decisions. For readers, plot is only revealed through narrative, but for authors, the relationship is often reversed: they begin by constructing a sequence of plot points and overlapping character arcs, then use narrative to build and connect those points in text. This top-down style of writing is often aided by tools like outlines, character sheets, and mind-maps \cite{zhaoMakingWriteConnections2025}, which let writers externalize and iterate on plot-level decisions before committing to more specific details like narrative voice and prose. 
% In this style of writing, plot points play a role analogous to that of keyframes in animation; they act as fixed points of reference from which the intervening material will be derived. However, unlike animation keyframes, plot points and character arcs cannot simply be interpolated---they must be told in a narrative voice. This 

% We build on this analogy by introducing \newterm{narrative keyframes}—high-level representations of story events and character arcs that specify the intended progression of a narrative. Our system uses these keyframes to generate text segments with distinct narrative goals, which users can iteratively recombine and refine to shape pacing, focus, and characterization.


% develop a narrative that reveals and connects them. This top-down approach to writing lets authors plan and revise story structure before committing to prose. 
% By mapping out causal dependencies, character motivations, and the timing of revelations in advance, they can iterate on high-level decisions that would otherwise require costly rewrites. It also facilitates techniques like foreshadowing and thematic resonance by allowing early passages to be written with knowledge of later developments. 

% In this sense, plot points function much like keyframes in animation: fixed reference points that define essential moments, with intervening material crafted to connect them smoothly and meaningfully. We build on this analogy by introducing \newterm{narrative keyframes}—high-level representations of story events and character arcs that specify the intended progression of a narrative. Our system uses these keyframes to generate text segments with distinct narrative goals, which users can iteratively recombine and refine to shape pacing, focus, and characterization.

% A key advantage of narrative keyframes is their support for perspective-based recombination. Users can generate multiple first-person accounts of the same events, capturing how different characters experience the same plot elements. Aspects of these perspective-specific narratives can then be used to condition the generation of a unified third-person account, helping authors control and balance characterization across the story.
% \tabref{tab:keyframing_example} illustrates this idea with a simple example, showing how first-person perspectives on the same event can be selectively recombined into different third-person characterizations.

% We present a system that operationalizes this framework. In our system, narrative keyframes are instantiated as character keyframes tied to plot points, while generated first-person perspectives serve as narrative realizations of those keyframes. The system allows writers to define character development through keyframes, compare multiple first-person perspectives on shared plot points, and synthesize selected character evidence into a unified third-person narrative. We evaluate the system through both a technical evaluation and a user study. Our technical evaluation, using both automatic and expert assessments, shows that stories produced with our framework have higher overall quality and richer characterization than those generated by a vanilla LLM baseline. 
% Results from our user study with 12 writers further demonstrate that narrative keyframing supports a more controllable, transparent, and engaging creative writing experience with generative AI, and better helps users control, manifest, and trace characterization in their stories than a chatbot baseline.

% The structure of creative text is often discussed at three different levels: first, a \newterm{story}, which broadly represents the collection of events and details included in a work; second, a \newterm{plot}, which traces a path of cause and effect through the events in a story; and third, a \newterm{narrative}, which represents how the plot is constructed and conveyed, including decisions that control pacing, focus, and characterization \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}.\footnote{The terms "story", "plot", and "narrative" are often used interchangeably in casual use, but we adhere to the more specific academic definitions to avoid ambiguity.} 
% Factoring creative text in this way can help us understand the structure behind creative decisions. For example, the same events (story) can be described in a different order (plot) and from different perspectives (narrative) to achieve different creative goals. In most cases, the reader comes to understand story and plot only through narrative. However, authors often create these elements in the opposite order by first constructing a story and plot, then using these to guide the construction of a narrative.

% Creative writing is often discussedd at two different levels: \newterm{plot}, which includes the basic facts of a story, how those facts are connected, and the order in which they are revealed; and \newterm{narrative}, which represents how the plot is revealed to control pacing, focus, and characterization \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}.
% % \footnote{The terms "plot", and "narrative" are often used interchangeably in casual use, but we adhere to the more specific academic definitions to avoid ambiguity.} 
% Deconstructing stories in this way can help us understand the structure behind creative decisions. To a reader, plot is only developed and revealed through narrative. However, authors often build these elements in the opposite order by first planning out plot points, and then building narrative to develop and connect those points in the final text.

% narrative is what reveals and develops plot; but for many authors, , authors often create these elements in the opposite order by first constructing a story and plot, then using these to guide the construction of a narrative.

% For example, the same events (story) can be described in a different order (plot) and from different perspectives (narrative) to achieve different creative goals. In most cases, the reader comes to understand story and plot only through narrative. However, authors often create these elements in the opposite order by first constructing a story and plot, then using these to guide the construction of a narrative.



% each new level of the story represents a world,  of decisions that control pacing, focus, and characterization.





% \abe{(possible for related work) Much has been said about creative writing, with academics discourse \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}}

==> sections/notes/oldintro.tex <==
\noindent{}Creative writing is often discussed at two complementary levels: \newterm{plot}, which encompasses the core events of a story, their causal relationships, and the order in which they occur; and \newterm{narrative}, which governs how those events are presented to shape pacing, emphasis, and characterization \cite{balNarratologyIntroductionTheory2004,genetteNarrativeDiscourseEssay1990,forsterAspectsNovel1927}. Distinguishing between these levels provides a useful lens for analyzing the structure underlying creative decisions. For readers, plot is only accessible through narrative. For authors, however, the relationship is often reversed: they first construct a sequence of plot points, then develop a narrative that reveals and connects them.

This top-down approach to writing lets authors plan and revise story structure before committing to prose. By mapping out causal dependencies, character motivations, and the timing of revelations in advance, they can iterate on high-level decisions that would otherwise require costly rewrites. It also facilitates techniques like foreshadowing and thematic resonance by allowing early passages to be written with knowledge of later developments. In this sense, plot points function much like keyframes in animation: fixed reference points that define essential moments, with intervening material crafted to connect them smoothly and meaningfully. We build on this analogy by introducing \newterm{narrative keyframes}—high-level representations of story events and character arcs that specify the intended progression of a narrative. Our system uses these keyframes to generate text segments with distinct narrative goals, which users can iteratively recombine and refine to shape pacing, focus, and characterization.

A key advantage of narrative keyframes is their support for perspective-based recombination. Users can generate multiple first-person accounts of the same events, capturing how different characters experience the same plot elements. Aspects of these perspective-specific narratives can then be used to condition the generation of a unified third-person account, helping authors control and balance characterization across the story.
\tabref{tab:keyframing_example} illustrates this idea with a simple example, showing how first-person perspectives on the same event can be selectively recombined into different third-person characterizations.

We present a system that operationalizes this framework. In our system, narrative keyframes are instantiated as character keyframes tied to plot points, while generated first-person perspectives serve as narrative realizations of those keyframes. The system allows writers to define character development through keyframes, compare multiple first-person perspectives on shared plot points, and synthesize selected character evidence into a unified third-person narrative. We evaluate the system through both a technical evaluation and a user study. Our technical evaluation, using both automatic and expert assessments, shows that stories produced with our framework have higher overall quality and richer characterization than those generated by a vanilla LLM baseline. 
Results from our user study with 12 writers further demonstrate that narrative keyframing supports a more controllable, transparent, and engaging creative writing experience with generative AI, and better helps users control, manifest, and trace characterization in their stories than a chatbot baseline.

==> sections/y-acknowledgement.tex <==
\begin{acks}

\end{acks}
